Machine Learning Research Towards Combating COVID-19: Virus Detection, Spread Prevention, and Medical Assistance

COVID-19 was first discovered in December 2019 and has continued to rapidly spread across countries worldwide infecting thousands and millions of people. The virus is deadly, and people who are suffering from prior illnesses or are older than the age of 60 are at a higher risk of mortality. Medicine and Healthcare industries have surged towards finding a cure, and different policies have been amended to mitigate the spread of the virus. While Machine Learning (ML) methods have been widely used in other domains, there is now a high demand for ML-aided diagnosis systems for screening, tracking, and predicting the spread of COVID-19 and finding a cure against it. In this paper, we present a journey of what role ML has played so far in combating the virus, mainly looking at it from a screening, forecasting, and vaccine perspectives. We present a comprehensive survey of the ML algorithms and models that can be used on this expedition and aid with battling the virus.

==> Revising-Old_Notes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%OLD-INTRODUCTION%

In December of 2019, a virus was discovered in Wuhan, China. A type of SARS-CoV-2 virus now referred as COVID-19 \cite{latif2020leveraging}. This respiratory virus has spread quite rapidly across the world was declared a global pandemic by March 2020 by World Health Organization (WHO) \cite{al2020asymptomatic}. At the time of writing this the total number of confirmed cases worldwide are over 10 million \cite{googlenews}.  
There has been significant research done by the scientific community since December 2019, an estimate of 100,000 papers have been published over a broad range of topics like testing, healthcare services, pathogenesis, structure of the virus, etc \cite{natureIndex}. 

In this survey paper we predominantly explore the research that has been conducted in Machine Learning (ML) concepts, algorithms and models related to COVID-19. We also provide a review on the research that has is related COVID-19 and Socioeconomics.

\textit{First,} we explore the research and potential contributions ML has in healthcare and medicine industries prior to COVID-19; research in epidemiology using ML algorithms suggest that ML algorithms can be integrated with statistical analysis and be used as a toolbox to better make sense of electronic health data  \cite{wiens2018machine} \cite{mou2019artificial} \cite{mak2019artificial}. Traditionally it is common practice in medicine to have data-driven analysis, however, with the integration of ML models can rapidly generate predictive results for questions that and symptoms that are common \cite{rajkomar2019machine} \cite{chen2017machine}. 

\textit{Second,} we review ML research done over historic epidemics such as SARS and MERS, these historic epidemics have previously infected humans too ; it is worth exploring whether ML research conducted over historic epidemics would aid in present day research. 

\textit{Third,} we review the topic on hand and review ML related research that has been conducted in predicting the spread of COVID-19, how ML algorithms and models could forecast the spread at a high accuracy and how textual analysis over social media posts can give an insight of the public sentiment.

\textit{Fourth,} ML has the capability in assisting healthcare workers by aiding in speed testing and diagnosing compared to the traditional Reverse Transcription Polymerase Chain Reaction (RT-PCR) which can take up to 2 days in diagnosing \cite{mei2020artificial}; ML algorithms have been previously been used for image analysis in X-Rays and CT Scans in determining lung nodules, cancer and even brain diagnosis \cite{suk2017deep} \cite{huang2017lung}. We explore how ML algorithms can aid healthcare workers in detecting COVID-19 using such image classification models.

\textit{Fifth,} we review how there is still a shortage of any potential drug or vaccine that can fight the virus \cite{boldog2020risk} \cite{shereen2020covid}; we review the research of ML algorithms and models that is done over vaccine development. There are no present drugs that are available to fight the virus either \cite{zhou2020network} so it is essential to see whether current drugs could be re-purposed and whether ML can aid in that process.

\textit{Sixth,} we review the research that has been done over seeing how the coronavirus has impacted society and the social and economic impact is has had \cite{torales2020outbreak} \cite{fernandes2020economic}.

\begin{table}[h!]
\caption{\label{tab:table-name}The Organization of the Paper.}
\centering
 \begin{tabular}{|m{1.0cm} | m{8em} | m{4cm}|} 
 \hline
 \textbf{Section} & \textbf{Title}  & \textbf{Description} \\ [0.5ex] 
  \hline
1 &  ML in Healthcare &  Recent finding in ML related to Healthcare and medicine \\
 \hline
2 &  Historic Epidemics &  Research covering ML related to studying previous epidemics \\
 \hline
3 &  Prevention and Spread &  Role of ML in predicting the spread of the pandemic \\ 
 \hline
4 & Diagnosis &  Role of ML in diagnosing COVID-19  \\ 
  \hline
5 &  Vaccine and Patient Recovery & The role of ML in finding a potential cure \\
  \hline
6 &  Social Impact & The socioeconomic impact of COVID-19 \\
 \hline
 \end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{The role of ML in Healthcare and Medicine}
ML algorithms are increasingly being implemented for patient care and multiple other clinical domains. The results of utilizing ML algorithms and techniques aids healthcare workers in diagnosis, clinical care and decision making, etc. \cite{ahmad2018interpretable}. The healthcare and medicine industries are at the forefront of doing their research on how ML can be implemented \cite{deo2015machine} \cite{maity2017machine}. In epidemiology ML technology can really aid in infectious disease control and transmission pathways \cite{kourou2015machine}, to combating cancer ML classification models can be employed towards classifying cancerous genes \cite{asri2016using} \cite{parmar2015radiomic} \cite{tan2003ensemble} \cite{shafai2019dose}. For diabetes ML models and methods can be used for diagnosis \cite{kavakiotis2017machine}. In this section we do a short review of the research and examples of ML in these industries.


% For clinical care ML base models provide an ease of querying relevant data from clinical records or by perhaps even auto-populating data fields in a form from clinical notes \cite{ross2019artificial}, the integration of ML for easing the administrative task and workflow can aid in reducing the physicians time spent on electronic health records which can take a physician's 49\% of the time whereas giving clinical time to their patients is only 33\%. Having ML-enabled tools may increase the staff productivity any where between 30\% and 50\% \cite{hazarika2020artificial}.

\indent ML has assisted in the healthcare and medicine sector by contributing significantly towards medicine, epidemiology, medical operations, and diagnosis\cite{allam2020artificial} of diseases using medical images. ML has really aided health professional over diagnosing patients using CT-Scans, MRIs and X-rays to detect anomalies \cite{wong2019artificial01} \cite{ards2019artificial} \cite{denecke2019artificial} \cite{van2017fifty} \cite{hawkins2016predicting}, we later discuss this in \textit{Section 04 - Diagnosis}).

There are a lot of studies in how ML can aid in diagnosing cancers, Artificial Neural Networks (ANN) can be used in diagnosing cancer cells in a lung in a study done by \cite{denecke2019artificial} where they have trained and validated a models. Similarly another ANN model is utilized in the research towards pancreatic cancer in a study by \cite{muhammad2019pancreatic} - addressing that there are preexisting routes to diagnosing pancreatic cancer, however, they can be very costly in some cases. Utilizing an ANN model may be a more feasible option on many fronts such as implementation and cost.\indent There are examples of studies and research done using AI and its' subset towards detection of breast cancer \cite{lamy2019explainable}. In a study done by \cite{rodriguez2019detection} reviews how a deep learning model network, along with image analysis algorithms and features classifications are to determine the suspicion of the cancer. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Role of AI in combating historic epidemics}
Before the novel COVID-19 (SARS-CoV-2) there have been other viruses and epidemics that have occurred. Other coronaviruses like Severe Acute Respiratory Syndrome (SARS-CoV) and Middle East Respiratory Syndrome (MERS). In a study done by \cite{jang2016comparison} the authors implement ML techniques such as Support Vector Machine and Decision Trees to determine the similarities between SARS and MERS, determining even though they are of the same family of viruses they are different. That continues to a research conducted recent to determine how there are a lot of similarities between pathogens and exposure between SARS and COVID-19 \cite{liu2020reproductive}. In this section we explore the research and studies that have been done in ML with respect to the previous corona-viruses.


\subsection{Severe Acute Respiratory Syndrome - (SARS-CoV)}
In 2002 China a disease known as the SARS-CoV was discovered. This disease caused patients to show flu like symptoms, respiratory problems, and was also transmitted person-to-person. SARS had been transmitted to 29 countries, likely infecting 8,098 cases worldwide with over 700 deaths according to WHO \cite{stadler2003sars}. As SARS-CoV shows a similar pattern to COVID-19 (SARS-CoV-2) the research relating to that could be helpful. In this section we give a quick overview of the research that had been done using ML to combat SARS.


\subsection{Middle East Respiratory Syndrome - (MERS-CoV)}
The coronavirus family has the capacity to penetrate into new hosts causing severe disease. First it was discovered in Saudi Arabia. MERS diverges from SARS in genome sequence the authors in \cite{turki2016greedy} highlight how the MERS-CoV respiratory does have a relatively high-rate of death. This was stated before COVID-19, of course. In this section we explore what time of ML techniques and models had been utilized at the time of the MERS outbreak.

ML techniques in this study were done to determine the morality rate of patients using a Greedy-Based Oversampling Approach (GBOA) using classification algorithms such as Random Forest and Support Vector Machines - in their findings they discovered that comparing with the standard approach their accuracy had the highest accuracy. \indent \cite{hong2017epidemiological} do a research where they compare neural network and support vector machine algorithms to conclude whether they could be conducted in epidemiological studies. 
\cite{sandhu2016intelligent} focuses on the geographical location of affected patients and the importance of it - using a Bayesian belief system over a cloud computing system could provide a risk assessment feature to control the outbreak. Cloud computing is utilized to share the data that is necessary. 
In a study done by \cite{choi2017large} ML techniques are utilized to attain an in-depth analysis to determine the public outlook and response to MERS over social platforms like Twitter and Facebook.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Prevention, the Spread - COVID19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Machine Learning algorithms can be implemented for predictive analysis, algorithms to predict consumer behavior, speech and input recognition are all examples of using ML technology like additive models, Bayesian Classifier, Decision Trees, and Spare Linear Models \cite{rai2020explainable}. ML classifier Naive Bayes Classifiers have a high accuracy in predicting heart-attacks in patients who have shown symptoms \cite{mastoli2019machine}. 

\begin{figure}[ht]
\centering
    \includegraphics[scale=.50]{images/March_Cases.png} 
    \caption{\cite{googlenews} \textit{Total number of on the day of declaring COVID-19 as a global pandemic.}}
    \label{fig: 1}
\end{figure}


\indent In this section we explore whether such algorithms and tools might be used in preventing the further spread of the current problem at hand, COVID-19 - this section is divided in the following sub-sections:

\begin{enumerate}[label=\Alph*.]
\item Early Tracking, preventing the spread
\item Forecasting - further spread
\item Applications and Text Analysis
\end{enumerate}

\subsection{Early Tracking, preventing the Spread}
We explore how ML algorithms might be able to predict the pandemic we are facing right now, such algorithms and models had already utilized to predict the rapid spread of COVID-19. 

In fact, prior to the WHO discovering and releasing official statements and warnings about the virus there were a few companies and laboratories that were able to predict its' possible threat.

Companies such as \textit{BlueDot} \cite{naude2020artificial} \cite{mccall2020covid} \cite{tuite2020estimation} \cite{long2020role} and \textit{Metiodata} \cite{allam2020artificial}  were amongst them. \textit{BlueDot} sourced data from news reports, previous data on animal disease outbreaks and airline tickets information they were then able to use their ML tools to predict that there will be definite outbreak occurring within other cities and regions of China \cite{allam2020artificial}. \textit{BlueDot} had warned its' clients about the outbreak on the 31st December 2019, almost over a week prior to the WHO making any statements about it \cite{naude2020artificial}. \newline
\textit{Metabiota} too used data and analytics to determine the spread of COVID-19, by using airline flight details of passengers they were able to successfully predict the outbreak in other countries like Taiwan, South Korea, Thailand, and Japan days prior to it actually happening \cite{allam2020artificial}. 



\subsection{Forecasting - Further Spread}
\indent It is important to predict and determine how the virus is going spread further across cities, and countries. Using AI to do this has been possible by utilizing techniques like clustering, support vector machine and data augmentation, etc.. Such techniques are explained in this sub-section.

Using a Modified Auto Encoder to train a model to predict the number of cases cities might have, the artificial neural network uses unsupervised learning technique along with k-means algorithm to attain a high level of accuracy in predicting the number of cases compared to the actual number of cases on a set date \cite{hu2020artificial}. 

Using Non-Auto Regressive Neural Network by utilizing recently history data is explained in \cite{ghazaly2020novel}, however, the scarcity of data at the time of their research does create a prediction error - concluding this method of AI might be efficient on other regression problems rather than for forecasting COVID-19. 

A model inspired by a previous methodology that was able to successfully forecast season influenza in the US at state level, along with the integration of previous methods to monitor emerging outbreaks is discussed in \cite{liu2020machine} - using a system called Augmented ARGONet to produce a 2-day forecast for clustered Chinese provinces; Approaching it from a data-driven mindset and utilizing the data from Chinese CDC, COVID-19 Baidu and other sources.

\cite{fong2020finding} addresses the importance of early forecasting, and how due to the epidemic there will be a scarcity of data. Addressing the challenges of data augmentation and different method of grouping data and structures. Implementing \textit{GROOMS} through a range of forecasting methods such as \textit{classical time-series forecasting, to self-evolving polynomial neural networks (PNN) and to working under panel sector.}


In the paper, research conducted by \cite{bandyopadhyay2020machine} - a Recurrent Neural Network is utilized with considering the accuracy and the RMSE (root-mean-square-error; a standard performance measure used for time series forecasting purpose.) as a metric to determine the algorithms performance. The architecture of RNN allows both sequential and parallel information processing, a close way to simulate how operations run in a human brain. Mixing that with Bidirectional RNN (BRNN) accesses the context of both future and past - LSTM (Long short-term memory) allows better long-range dependencies and GRU (Gated Recurrent Unit) control the information inside the unit.

To determine the correlation between the temperature and rising number of cases \cite{siddiqui2020correlation} is done through the machine learning k-means Clustering algorithm. With the objective to analyze the effect of the COVID-19 cases including, suspected, confirmed and death cases. By this algorithm it is possible to predict the cases in a specific country or area and we can prevent travelling.
\begin{figure}[ht]
\centering
    \includegraphics[scale=.50]{images/June_cases.png} 
    \caption{\cite{googlenews} \textit{Total number of cases at the end of June 2020.}}
    \label{fig: 2}
\end{figure}
\subsection{Applications and Text-Analysis}

% Similarly, the use of mobile applications with the use of ML technology can collect real-time data that can utilizes these algorithms to create a map of the patients condition allowing doctors and nurses to be more attentive and alert \cite{lopes2020predictive}. 


With majority of the population having a smart phone \cite{luther2005enhanced} and applications that can track a users habits and movements \cite{stawarz2015beyond}. Use of in App location services, and reminders on these apps may have become and integral part of our day-to-day lives. In this section we explore how we use of applications and the integration of ML could assist during this pandemic.

\cite{rao2020identification} AI algorithms integrated with phone-based online survey to deduce whether the individual need to be isolated or not. The online survey is used as a medium of collecting data, these data points go through a framework which evaluates and groups the individual on whether they are at no risk, moderate risk, and high risk groups - by getting this immediate feedback it would allow individuals to isolate and socially-distant themselves. The survey is based on general information about the individual on where they might be located, their demographic, recent travel history or encounters with anyone who may have tested positive, and then using a check box to record any signs and symptoms that might be shown by the individual.

%%%%%%Potential Text Analysis Section As its' own

Twitter has become a form of blogging and updates, its' users can constantly use the app to check news and validate alerts. The study done by \cite{jahanbin2020using} gathers data that use relevant hashtags, upon text-cleaning or filtering the data, the tweets are processed through classification algorithm called Eclass1-MIMO.
Doing this can give us understanding over the morbidity rate in regions.

Similarly, using data from Twitter is addressed in the research done by \cite{samuel2020covid} - addressing how during the pandemic people turn to social media to raise their concerns and can be socially more active about it, hence, having a showing sentiment towards the situation. The research covers details on how \textit{Natural Processing Language, Textual Analysis, and Sentiment Analysis} are done using key phrases and words. Using Machine Learning Algorithm the authors are able to classify the increase towards negative and fearful sentiment from the public. The analysis aids in giving an early insight on the generic attitude of the public and ideally be able to give a guidance for policy makers to make decisions on how to communicate better with the public with this ever-growing pandemic.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%555
A sentiment analysis is also done by \cite{prabhakar2020informational} - addressing the need for it as there is a potential of misinformation being spread across social platforms. The use of Latent Dirichlet Allocation (LDA) an unsupervised algorithm is done to spot the semantic relationship between words.

The use of another social platform \textit{Sina-Microblog} is used to express raising concerns in China. Authors in \cite{zhao2020chinese} gather data from the blog and analyze it using methods such as word segmentation, word frequency, and sentiment analysis. The authors are able to build a visual cluster highlighting the public opinion over the pandemic. 

Since the emergence of the virus there has been a lot of Sinophobic behavior across web platforms and social media - the research done in \cite{schild2020go} utilizes data from Twitter and 4Chan. The study sees interesting differences and opinions towards the Chinese population before and after COVID-19. Using a shallow neural networks to create a model that put context to the word that is being used, this is done by training multiple word2vec models.

\begin{table*}[h!]
 \caption{\label{tab:table-name}Predictive Analysis Tools and Methods.}
 \centering
\begin{tabular}
{|m{1cm} | m{3.25cm} | m{4cm}| m{7cm}|}  
\hline
  \multicolumn{1}{|c|}{\textbf{Reference}}&
  \multicolumn{1}{|c}{\textbf{Sections}}&
  \multicolumn{1}{|c}{\textbf{Model and Technology}}&
    \multicolumn{1}{|c|}{\textbf{Description and Limitation}}
  \\\hline
\cite{allam2020artificial}  &
  \multirow{2}{*}
  {Early Tracking, Prevention}
 & Predictive Analysis tool & Using flight details data annd recent outbreaks to predict the spread in nearby countries\\\cline{3-4}\cline{1-1}
\cite{hu2020artificial} &     &  ANN - K-Means Algorithm & Using a MAE to successfully predict 2-day spread  \\\cline{3-4} \hline
\cite{ghazaly2020novel} &
  \multirow{5}{*}
  {Forecasting}
 & Non-Auto Regressive Neural Network & Prediction Error, due to scarcity of error at the time of Analysis \\\cline{3-4} \cline{1-1}
\cite{liu2020machine} &     &  Augmented ARGONet & Clustering of Chinese Provinces, and getting a 2-day forecast\\\cline{3-4}\cline{1-1}
\cite{fong2020finding} &     &    Polynomial Neural Network (PNN) - GROOMS & Addressing data augmentation and importance of early forecast \\\cline{3-4}\cline{1-1}
\cite{bandyopadhyay2020machine} &     &   RNN & Researching predicting using GRU + LSTM combined models \\\cline{3-4}\cline{1-1}
\cite{siddiqui2020correlation}  &       &  K-Means Clustering Algorithm &   Possible to predict the spread of cases \\\cline{3-4}\cline{1-1}
\hline
\cite{rao2020identification} &
  \multirow{6}{*}
  {Tracking and Text Analysis}
 & AI Algorithms & Phone based survey to determine whether a person is high-risk, low-risk or contracting the virus \\\cline{3-4}\cline{1-1}
\cite{jahanbin2020using} &     &    Eclass1-MIMO   & Classifying a twitter dataset to determine morbidity in regions \\\cline{3-4}\cline{1-1}
\cite{samuel2020covid} &     &  Natural Processing Language   & Getting public sentiment by classifying tweets \\\cline{3-4}\cline{1-1}
\cite{prabhakar2020informational} &     &  Latent Dirichlet Allocation (LDA) & Algorithms used to spot semantic relationship between words \\\cline{3-4}\cline{1-1}
\cite{zhao2020chinese} &     &  Sentiment Analysis   & Building a visual cluster to highlighting public opinion over pandemic \\\cline{3-4}\cline{1-1}
\cite{schild2020go} &     & Shallow Neural Networks & Training multiple word2vec models to put context to words\\\cline{3-4}\cline{1-1}
\hline
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The role of ML in Diagnosis - COVID19}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typically COVID-19 is confirmed by conducting the reverse-transcription polymerase chain reaction (RT-PCR). However the sensitivity of this test is not enough to detect the disease in early stages and more over there is cost involved in conducting the test. 
% Computed tomography (CT) is a non-invasive imaging approach, which can detect certain characteristics in the lungs associated with COVID-19 patients. 
% As some COVID-19 CT may share some other characteristics that might belong to pneumonia. It is impossible for a technician to keenly observe all the features and then make a decision. In these times of high volume of patients, practically going through all the CT scans is a tedious process.
% In this section we go over the rapidly developed ML-Based automated image analysis tools that can be used to get high accuracy in detecting Corona virus positive patients as well as quantification of disease burden.

The virus enters through the respiratory system, infecting the lungs \cite{santosh2020ai} \cite{ozkaya2020coronavirus} \cite{pan2020time}. Some patients might show symptoms, where as some may be asymptomatic - hence, diagnosing the virus as early as possible is essential. Integrating ML into the the diagnosis stage could really assist the healthcare workers \cite{bullock2020mapping}. It is important to explore this as an alternative to standard testing as it would speed up the process but also aid to countries where majority of the population does not have intensive care \cite{gosai2020digital} \cite{pham2020artificial}.

\begin{figure}[ht]
\centering
    \includegraphics[scale=.40]{images/X_Ray_COVID.JPG} 
    \caption{\cite{el2020covidx} \textit{Shows a comparison between a regular Chest X-Ray to an X-Ray that is infected by the virus.}}
    \label{fig: 3}
\end{figure}

\indent In this section we explore primarily towards the diagnosis of COVID-19 by reviewing the research that has been done over ML Image classification Models on traditional X-Ray Images and CT Scans - utilizing image classification models to diagnose whether a patient may have the virus or not.

Recently, using deep learning has demonstrated a great success in medical imaging due to its high capability of feature extraction. In the paper \cite{li2020artificial} they discuss about the three-dimensional deep learning framework to get more accuracy. Analysis of such images can aid the health care workers in diagnosing the patients and see whether they might be COVID-19 positive or negative, or perhaps even the likely-hood of severity if they are positive \cite{zhao2020covid}.

Discussing the ML algorithms that are being developed for nucleic acid detection assays that are comprehensive across the genomics diversity and the prediction is highly accurate in \cite{metsky2020crispr}.

In order to utilize various ML models and algorithms it is important to train the models with preexisting data - Machine Learning algorithm that have been properly trained can help interpret the X-rays and CT scans in seconds and health workers can work on the actual job on the instead of interpreting the data\cite{zhang2020covid} \cite{wang2020covid} \cite{apostolopoulos2020covid} \cite{shan2020lung}.

A model that has been implemented is quite high in detecting severity of a COVID-19 Case \cite{tang2020severity}. Implementing automatic severity based on Random Forest (RF), taking into account several characteristics, classifies the COVID-19 severity in case. Using Binary Classification to decide whether it is an extreme case or not, this is also a drawback as the model does not classify the intermediate cases as COVID-19 can be triggered, normal or even without symptoms.

The current infrastructure for detecting the positive patients is becoming a difficult task as there is not enough data to train the machine learning algorithms. Deep learning models usually tend to ma

ke over confident predictions, however, \cite{ghoshal2020estimating} has an objective to achieve the state-of-the-art performance but to evaluate the uncertainty by using Bayesian Convolutional Neural Networks(BCNN) in conjunction with drop weights to improve the diagnostic performance.

2D and 3D deep learning models are deployed and multiple retrospective experiments are are conducted to analyze the performance of the system. The program produces a "Corona Rating" involving all these functions. Based on the score it is possible to take a decision\cite{gozes2020rapid}.

 \begin{table*}[h!]
\centering
  \caption{\label{tab:table-name} Data Sets, Sources, Methods and Performance.}
  \begin{tabular}{|m{1cm} | m{1.5cm} | m{3cm}| m{4cm} | m{5cm}|}  
 \hline
 \textbf{Image } & \textbf{Ref} & \textbf{Dataset} & \textbf{Methods} & \textbf{Remarks} \\ [0.5ex] 
 \hline

  \cite{apostolopoulos2020covid} & \multirow{2}{*}{X-Ray} &  Multiple curated Datasets \textit{source: Github} & DL - CNN, Feature Extraction (various models) & Various model performance comparison  \\ \cline{1-1}\cline{3-5}
 \cite{ghoshal2020estimating} &                   & Publicly Available Chest X-Ray & Bayesian CNNs & Accuracy of 89.92 Percent \\  \cline{1-6}
 \hline
 \cite{zhao2020covid}  & \multirow{12}{*}{CT-Scan} & Open-sourced COVID-CT \textit{source: Github} & multi-task and self-supervised learning & Clinically useful, achieving accuracy of 89 percent.   \\ \cline{1-1} \cline{3-5} 
  \cite{tang2020severity} &                   & Clinical CT Images of 176 & Random Forest / three-fold cross-validation & 87.5 Accuracy  \\ \cline{1-1} \cline{3-5}
 \cite{gozes2020rapid} &                   &   Multiple Datasets \textit{Multiple Source: Hospitals / Chainz} & Deep Learning Image Analysis & Various, over 90 percent mostly \\ \cline{1-1} \cline{3-5}
  \cite{li2020artificial} &                   & Independent Dataset CT Images & Deep Learning mode - Detection Neural Network & 96 percent in detecting C-19  \\ \cline{1-1} \cline{3-5}
    \cite{butt2020deep}  &                   &  Clinical CT Scan Images & Deep Learning - ResNet & Accuracy of 86.7 percent  \\ \cline{1-1} \cline{3-5}
    \cite{wang2020deep} &                   &   CT Scan Images Dataset, Clinical &  Modified Transfer Learning & 79.3 Percent Accuracy  \\ \cline{1-1} \cline{3-5}
     \cite{bai2020predicting} &                   &  China Health Commission Dataset, etc & Traditional Multi Stage - Deep Learning Methods & AUC 0.954  \\ \cline{1-1} \cline{3-5}
      \cite{jin2020development}  &                   &  Clinical / Hospital & Deep-Learning Model & AUC 0.97    \\ \cline{1-1} \cline{3-5}
       \cite{jin2020ai}  &                   &  Hospitals & Deep-supervised encoder, 3D U-Nett++ & Sensitivity 0.974\\ \cline{1-1} \cline{3-5}
        \cite{shan2020lung}  &                   &   Clinical & Deep Learning - vB-Net & High Accuracy \\ \cline{1-1} \cline{3-5}
      
  \cite{zheng2020deep} &                   &  Clinical & Deep Learning Models  & AUC 0.975  \\  \cline{1-6}
  \hline
 \end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The role of AI in Vaccine Development and Patient Recovery - COVID19}
%%%%%%%%%%%%%%%%%%
Maximizing the advancements in the computational power and the machine learning algorithms there has been a lot of research in development of drugs and medicines, and drug repurposing \cite{napolitano2013drug}. In this section we explore the research that has been done with respect to the Machine Learning algorithms related development of a vaccine for COVID-19 or repurposing of drugs that are available to mitigate the severity of the illness.

\begin{enumerate}[label=\Alph*.]
\item Vaccine Development
\item Drug Re-purposing
\end{enumerate}
% The drug development and medicine industry has is where AI and its' subsets have been lauded for their work \cite{naude2020artificial2}.
\subsection{Vaccine Development}
With the fast and fatal spread of COVID-19, it has become an emergency and priority to find a vaccine that could provide immunity against COVID-19. In this section we explore ML techniques that can assist in possibility of creating a vaccine.

As highlighted by \cite{ong2020covid} that the creation of a vaccine is critical in controlling the spread of the virus and putting this to an end. Previously there have been animal cases who that have contracted the coronavirus or a type of it at least, hence, the vaccine production and research on this topic is being conducted for sometime. 
However, nothing concrete has been of conclusion with the safety and efficacy for human trials - hence, alternate methods rather than trials have to be conducted in the development for a vaccine. The use ML to compute the possible score of a protective immunity when the vaccine is induced by a candidate is conducted in this reasearch - utilizing the tool Vaxign to aid in development by using reverse vaccinology (RV). Using bioinformatics analysis of pathogen genomes. They used ML Classification algorithms such as logistic regression, Support Vector Machine, K-nearest neighbor, \textit{random forest}, and extreme gradient boosting (XGB) - these models were tested on a five-fold cross validation.

% In a research done by \cite{magar2020potential} they mention how due to not having enough data on biological structures and DNA/protein sequences ML can be used to predict biological structures and phenomena - using ML technique to predict to study how virus-antibody sequences and the patient neutralization response would be. It is important to have enough data to train the models, so techniques can be used in mapping between virus and the effectiveness of the synthetic antibodies. ML techniques can potentially simulate and learn how the anti-bodies will react with the immune system faster than the human immune system itself hence this model can act as a bridge in finding the most dependable one.

\subsection{Drug Re-purposing}
\cite{reda2020machine}
\cite{nguyen2020origin} addresses the origin of the virus in their study, understanding where it comes from and how it might be combated with - in their research they utilize unsupervised machine learning and computational biology to interpret the genomics sequences, this study could assist in finding the right drugs that could potentially stabilize or fight the virus.

% In the research conducted by \cite{yan2020prediction} they have used a machine learning model in order to predict the survival rate of critically ill COVID-19 patients. A prognostic machine learning model that was able to successfully predict the survival rate of patients, up to 90 percent. At a time where there's scarcity of data, this model only uses three clinical features - These three features represent tissue injury, immunity, and inflammation-typed indices - as a means of diagnosis this could seem low-cost and prompt critically. Using a XGBoost Machine Learning as it has a superb pattern characterization and feature selection ability. Method to establish the prediction model. 


ML models are being used as a discovery tool on the current FDA approved drugs and or compounds that are in the late stage for clinical trials for the effect of SARS-CoV-2 on human cells. \textit{To evaluate the specificity of the phenotypic profile to the impact of the virus we compared the effects of active SARS-CoV-2 to inactive ultraviolet-irradiated (UV-IR) and mock preparations of SARS-CoV-2 on cell} Using the neural networks to generate a high dimensional featurization of identification of each distinct phenotypic profiles \cite{heiser2020identification} - the results achieved in their paper, they were able to conduct analysis of over 1600 approved drugs in a human cellular model of SARS-CoV-2 infection.

A similar approach and method was conducted in the paper \cite{beck2020predicting} addresses the family of the virus, and how both SARS-CoV and MERS-CoV had a high morality rate and the need for the drug that would cure prevent had already prior existed but not yet fully found as it can take years, however, with SARS-CoV-2 (COVID-19) surfacing as a pandemic the need for a drugh has created even more of an urgency. Hence, perhaps re-purposing of the current available drugs is essential. In this study AI tools are used to explore how the drugs how this could be achieved and the MT-DTI (Molecule Transformer-Drug Target Interaction) model which is used to predict binding affinity values between the drugs that are available and target proteins. This type of self-attention mechanism has showed success in NLP Literature. This model is one of the best deep learning model to predict the affinity, however, this conclusion comes prematurely as there are still to be experimental evaluations to determine that. A form of DTI (Drug Target Interaction) models.

% A dataset called VirusNet which is based on data from previous viruses such as Influenza, HIV, SARS, Ebola, etc - the data is patient clinical and biochemical data. Usage of different classifier algorithms to determine whether anti-body would be capable of neutralizing the virus or not - algorithms such as XGBoost, Random Forest, Multi layer Perception, Support Vector Machine (SVM). 
% For this paper the province of Hubei is chosen as a case study. Maximum, minimum, average daily temperatures, town density, relative humidity, and wind speed are considered for this study. And for the 30days the number of reported cases is taken as the output dataset. There are a wide range of I algorithms that are used, they used GMDH algorithm in this paper. Regression analysis on the input data set was performed before binary classification of the GMDH algorithm \cite{pirouz2020investigating}.

\begin{table*}[h!]
  \caption{\label{tab:table-name} Vaccine and Drug Development }
\begin{tabular}
{|m{1cm} | m{3.25cm} | m{4cm}| m{7cm}|}  
\hline
  \multicolumn{1}{|c|}{\textbf{Reference}}&
  \multicolumn{1}{|c}{\textbf{Sections}}&
  \multicolumn{1}{|c}{\textbf{Model and Technology}}&
    \multicolumn{1}{|c|}{\textbf{Description and Limitation}}
  \\\hline
\cite{ong2020covid} &
  \multirow{2}{*}
  {Vaccine Development}
&  ML Algorithms Logistic Regression, Support Vector Machine, etc & Using a tool called Vaxign to implement Reverse Vaccinology \\\cline{3-4} \cline{1-1}
\cite{magar2020potential}  &       &    ML Techniques  & Simulating how anti-bodies will react to synthetic anti-bodies \\\cline{3-4}\cline{1-1}
\hline
\cite{heiser2020identification} &
  \multirow{2}{*}
  {Drug Re-purposing}
 & DL Models - Neural Networks  & Analysing how approved FDA Drugs would work against COVID-19 \\\cline{3-4}\cline{1-1}
\cite{beck2020predicting}  &     &   DL - Drug Target Interactions  &   Re-purposing current drugs to find out whether there is an affinity between drug and proteins \\\cline{3-4}\cline{1-1}
\hline
\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{The social impact of COVID-19, and how ML may assist with future pandemics}
COVID-19 is a present day global pandemic \cite{WHOC19}, it has been announced as a pandemic for over 12 weeks now and countries and cities have taken drastic measures to mitigate it. In this section we review how ML algorithms can predict the potential change in society and policies, and how the world has been impacted overall due to the virus.


The section has two subsections, listed below:
\begin{enumerate}[label=\Alph*.]
\item Socioeconomic impact of Coronavirus
\item AI integrated with the impact of Coronavirus
\end{enumerate}

\subsection{Socioeconomic impact of Coronavirus}
The world as a whole includes many components which they work in sync with each other, with plenty of trading between nations - an example could be used of building an automobile. That a European car may be manufactured in North America with parts that are shipped from Europe and assembled using tools that are manufactured in China. This is just one example, there is plenty of areas beyond manufacturing on how the world is so intertwined through supply chain. The authors in the study \cite{ali2020covid} use a metaphorical  example of a chain that is linked to and that could be the global supply chain, wherein, if a link of the chain is broken it might cause a form of hindrance. China the largest exporter in the world \cite{jiang2020research} was unfortunately the origin of the global epidemic i.e. COVID-19. To this date, with the virus being declared as a global pandemic there have already been changes implemented by many nations such as lock downs and shutting down businesses, travel and hospitality industries were among the ones that took a big hit. In these industries thousands of employees lost their jobs, or have been furloughed.\cite{nicola2020socio}


All these drastic changes would definitely leave an inevitable dent in the global economy, previously, when comparing to the prior pandemic SARS it is estimated that the global loss on the economy went then was as high as 40 Billion dollars \cite{evans2020socio}.

\subsection{AI integrated with the impact of Coronavirus}
Data is in abundance everywhere - even though there has been a change this recent pandemic has highlighted that its' not enough. It is understood that data is private, and maintaining its confidentiality and integrity is another aspect that most of us value - however, having said that, when it comes to health care and policies, the constraints and limitations need to be changed. In  study done by \cite{allam2020artificial} it is addressed that protocols need to be set by policy makers more so as cities move towards striving to becoming more smart it has been more so attainable to gather data such as location, and communication - this type of data can really assist in predicting more accurately which could lead to more rapid decision making and ideally in the case of pandemics, preventing them sooner. It is worth nothing that COVID-19 was predicted as a potential pandemic in a mere days compared to previous such as SARS it may have taken month \cite{allam2020artificial}.

Using the similar mindset a similar research is done by the authors in
\cite{allam2020coronavirus} to address the social
They studied data in this paper relating to four countries, USA, China, South Korea and Italy. The role of the Government's quarantine measures and isolation measures in reducing the pandemic's rapid growth. Generally neural networks are used with a number of parameters to approximate the nonlinear functions.They are powerful tools to approximate Quarantine effects in combination with the analytical epidemiological   models\cite{dandekar2020quantifying}.
Predicting future pandemic outbreak using AARIMA (Auto-Regressive Integrated Moving Average Model). Statistics of the Johns Hopkins University's total reported deaths was used in this paper to forecast the future scenario. Vector Auto Average (VAR) model is used with remote sensing data to estimate spatial extinction \cite{kumar2020forecasting}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
OLD ABSTRACT
% As of the writing of the paper COVID-19 has been declared a global pandemic. There have been millions of infected cases. It is has had a very high fatality rate, over a very short period of time. Everyone, globally, is doing their best efforts in finding a cure for the virus; nations across the world have enforced strategic social actions to reduce or contain the spread of the virus. In our comprehensive survey paper we take a journey in exploring how the research that has been carried out by Machine Learning (ML) community in tackling the virus. We present how ML has been in effect in aiding to the healthcare industries during to the pandemic, and how that may be implemented now.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[ht]
% \centering
%   \caption{\label{tab:table-name} ML Research done towards Diagnosing COVID-19.}
%   \begin{tabular}{|m{3cm} | m{1.5cm} | m{3cm}| m{4cm} | m{5cm}|}  
%  \hline
%  \textbf{Ref} & \textbf{Image Type} & \textbf{Dataset} & \textbf{Methods} & \textbf{Remarks} \\ [0.5ex] 
%  \hline

% \cite{apostolopoulos2020covid} & \multirow{10}{*}{X-Ray} &  Multiple curated Datasets \textit{source: Github} & DL - CNN, Feature Extraction (various models) & Various model performance comparison  \\ \cline{1-1}\cline{3-5}
% \cite{ghoshal2020estimating} &                   & Publicly available Chest X-Ray Images & Bayesian Deep Learning Classifiers & Using Transfer learning approach with the classifier to estimate uncertainty. \\  \cline{1-1}\cline{3-5}
%  \cite{farooq2020covid}, \cite{wang2020covid}, \cite{ucar2020covidiagnosis}, \cite{afshar2020covid}, \cite{luz2020towards}, \cite{khobahi2020coronet}, \cite{sarker2020covid}, \cite{hirano2020vulnerability}, \cite{hemdan2020covidx} &                   & COVIDx & Multiple prepossessing techniques like normalization integrated with various deep neural works and classifiers  & \begin{itemize} 
%  \item\cite{khobahi2020coronet} \cite{sarker2020covid} \cite{luz2020towards} \cite{wang2020covid} multiple approaches like semi-supervised approach, feature extraction and transfer learning methodology implemented.
%  \item\cite{ucar2020covidiagnosis} present an AI system that  classifies input of X-Ray images of Normal, COVID-19, Pneumonia using DL.
%  \item\cite{farooq2020covid} Use a ResNet classifier to achieve excellent classification accuracy.
%  \item\cite{hemdan2020covidx} Test and train multiple image classifiers to obtain the highest accuracy identifying the virus. VGG19 and DenseNet have a high accuracy score.
%  \item \cite{hirano2020vulnerability} Demonstrate how DNNs are vulnerable to a universal adversarial perturbation causing failure in classification tasks, fine-tuning may be able to improve this. 
%  \item \cite{afshar2020covid} An alternative modeling framework based on Capsule Networks.
% %  \item \cite{sarker2020covid} Clear explanation of how model works using a novel transfer learning approach 
%  \end{itemize} \\ \cline{1-1}\cline{3-5}
% \cite{narin2020automatic} &                   & Small Dataset available on GitHub & Three different CNN models (InceptionV3, ResNet50, Inception-ResNetV2) & ResNet50 provides the highest classification. \\ \cline{1-1}\cline{3-5}
% \cite{maghdid2020diagnosing} &                   & Multiple Sources & Modified Pre-trained AlexNet and a simple CNN & Pre-Trained network achieves a higher accuracy  \\ \cline{1-1}\cline{3-5}
% \cite{tougaccar2020covid} &                   & Multiple Sources and Datasets & MobileNetV2/SqueezeNet & They use DL models achieve high classification rate\\ \cline{1-1}\cline{3-5}
% \cite{ozturk2020automated} &                   & Multiple Sources  & DarkCovidNet (CNN) & Provides two approaches, a binary classification and multi-class classification. Binary model performs better and higher\\ \cline{1-1}\cline{3-5}
% \cite{rajaraman2020training} &                   & Multiple sources, datasets & VGG16, InceptionV3, Xception, DenseNet-121, NasNet-Mobile, etc models compared & VGG16 achieved the highest rate\\ \cline{1-1}\cline{3-5}
% \cite{jamil2020automatic} &                   & Kaggle Repository & Convolutional Neural Network & The authors are able to get 93\% accuracy \\ \cline{1-1}\cline{3-5}
% \cite{sethy2020detection} &                   & Multiple Datasets & Trained 9 different models for COVID-19 & ResNet50 + SVM achieved the highest accuracy\\ \cline{1-1}\cline{3-5}
% \cite{apostolopoulos2020extracting} &                   & Multiple Datasets & MobileNetV2 & Traininn the CNN MobileNetV2 model from scratch proves to get higher accuracy compared to transfer learning techniques  \\ \cline{1-6}
% \hline
%  \cite{zhao2020covid}  & \multirow{12}{*}{CT-Scan} & Open-sourced COVID-CT \textit{source: Github} & multi-task and self-supervised learning & Clinically useful.   \\ \cline{1-1} \cline{3-5} 
%   \cite{tang2020severity} &                   & Clinical CT Images of 176 & Random Forest / three-fold cross-validation & The Random Forest model showing promising performance towards reflecting the severity of COVID-19 \\ \cline{1-1} \cline{3-5}
%  \cite{gozes2020rapid} &                   &   Multiple Datasets \textit{Multiple Source: Hospitals / Chainz} & ResNet50 & High accuracy in identifying whether COVID-19 cases \\ \cline{1-1} \cline{3-5}
%   \cite{li2020artificial} &                   & Independent Dataset CT Images & Present a Deep Learning model CovNET & The model has the ability to high accuracy in identify COVID-19 cases from other lung diseases  \\ \cline{1-1} \cline{3-5}
%     \cite{butt2020deep}  &                   &  Clinical CT Scan Images & Deep Learning - ResNet18 & Using a location attention mechanism on the model distinguishes COVID-19 cases from others with higher accuracy \\ \cline{1-1} \cline{3-5}
%     \cite{wang2020deep} &                   &   CT Scan Images Dataset, Clinical &  Modified Transfer Learning - Inception Model & Use a fine-tuning technique with pre-trained weights \\ \cline{1-1} \cline{3-5}
%         \cite{bai2020predicting} &                   &  China Health Commission Dataset, etc & Multi Stage - DL Models, LSTM & The model is capable of extracting spatial and temporal information efficiently thereby improving prediction performance \\ \cline{1-1} \cline{3-5}
%       \cite{pathak2020deep}  &                   & Multiple datasets  & ResNet50 & The model with transfer learning technique performs better than alternative supervised learning methods \\ \cline{1-1}        \cline{3-5}
%         \cite{jin2020ai}  &                   &  Multiple sources: Hospitals & Various DL learning models (Inception, ResNet50, 3D U-Net++) & Able to deploy the model in 4 weeks overcoming challenges and achieving a high accuracy rate\\    \cline{1-1} \cline{3-5}
%         \cite{shan2020lung}  &                   & Clinical Dataset & Deep Learning - VB-Net & Introducing a Human-in the loop section to refine automation of each case - the model can segment and quantify infected regions\\ \cline{1-1} \cline{3-5}
      
%         \cite{zheng2020deep} &                   &  Clinical & UNet, Weakly Supervised DL Network (DeCovNet)  & Accurately predict COVID-19 infectious probability without annotating lesions for training  \\  \cline{1-6}
%   \hline
%  \end{tabular}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{The role of ML in Healthcare and Medicine}
% %Healthcare and Medicine industries makes use of the ML technology by implementing it for multiple clinical domains, these industries have been at the forefront of researching the integration of ML \cite{deo2015machine} \cite{maity2017machine}. 
% This section presents a short-review of ML technology integrated in healthcare to aid healthcare workers with diagnosis of diseases, %clinical care and decision making for patients 
% and by determining the role of ML in epidemiology.
% \cite{ahmad2018interpretable} \cite{allam2020artificial}. 

% Epidemiology is analyzing the risk factors for diseases that have a pattern to spread, it is identifying and predicting the distribution of determinants for a disease. Supervised ML models like regression modelling can be used to predict the outcome of a disease, and unsupervised models can be used to determine the patterns of a disease \cite{wiemken2020machine}. 
% There has been significant ML research in analyzing the spread of another contagious respiratory virus Influenza. Using the available clinical data on the virus along with the integration of ML models it can be possible to have early-warning ML models to predict an outbreak \cite{schmidt2019prediction}. The role of ML in Prediction and Forecasting COVID-19 is further discussed in \textit{Section 03 - Prediction and Forecasting of COVID-19}.

% An increasing number of studies have been dedicated towards using ML for diagnosis and prediction of diseases.
% ML models are vastly trained over a dataset consisting of medical images like CT Scan, MRI, or X-Ray to detect anomalies \cite{wong2019artificial01} \cite{ards2019artificial} \cite{denecke2019artificial} \cite{van2017fifty} \cite{hawkins2016predicting} \cite{parmar2015radiomic}. Classification models such as Support Vector Machine (SVM), Naive Bayes (NB), K-Nearest Neighbor (K-NN) can be implemented in diagnosing breast cancer and achieving a prediction accuracy of 97.13\% \cite{asri2016using} \cite{lamy2019explainable} \cite{shafai2019dose}. A similar approach can be used for diagnosis of lung cancer \cite{kadir2018lung}. The severity of cancer can be determined by using ML models like Clinical Tree, Random Forest and Logistic Regression models \cite{bergquist2017classifying}. The role of ML in Diagnosing diseases is further discussed in \textit{Section 04 - Diagnosis of COVID-19}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Role of ML in combating historic epidemics}
% Coronaviruses are a family of viruses that cause diseases in humans and animals, the present day pandemic COVID-19 (SARS-CoV-2) is a type of Coronavirus that belongs to that family \cite{nguyen2020origin}. Similarly, there are historical examples of coronaviruses that have affected humans. 
% Severe Acute Respiratory Syndrome (SARS-CoV) and Middle Eastern Respiratory Syndrome (MERS) are examples of such coronaviruses that were declared as epidemics \cite{song2019sars}. In this section we review ML research that is conducted over these viruses.

% SARS is a respiratory virus that was transmissible from person to person and it first identified in 2003. The virus had over 8000 confirmed cases worldwide during its' course that affected over 26 countries \cite{sarsnews}. SARS may also be referred as SARS-CoV, it is a predecessor to the present global pandemic COVID-19 (SARS-CoV-2). The two viruses belong to the same family of coronaviruses. People who contracted SARS showed symptoms like body aches, fever, fatigue, sore throat and etc., most of these are very similar to the symptoms that are shown by COVID-19 patients. Our objective was to review ML research done over SARS-CoV-1 that may have been resourceful for the current pandemic of COVID-19. Unfortunately, as SARS was identified and contained in 2003 we were unable come upon any ML research that would aid to this.

% First reported in Saudi Arabia in September 2012 \cite{mersnews}, MERS is respiratory virus that had a high fatality rate then. The infected patients showed symptoms ranging from cough, fever, pneumonia, etc. These similar symptoms are now shown by patients who are infected with COVID-19. As MERS was an airborne virus it could be transmitted through close contact a similar nature of transmitting to COVID-19, to date MERS has infected 2494 people across 27 countries \cite{merswho}. MERS also belongs to the same family of coronaviruses and as a result there are multiple commonalities between MERS and COVID-19 therefore any ML and MERS related exists could be helpful in the battle against COVID-19. 
% To control the spread of this easily transmittable virus communities were highly recommended to wear masks, stay home when possible, to wash hands, cover cough and sneezes, etc., almost all similar precautions that we as a society are now being asked to take for COVID-19. Epidemiological and ML approaches were also taken to control the spread of MERS, an example is the research conducted by Sandhu et al. \cite{sandhu2016intelligent} who create a ML model that utilizes GPS technology along with cloud computing power and Google Maps to represent potentially infected patients and provide an alternative route for uninfected users resulting in potentially mitigating the spread. The model reaches classification accuracy of 80\% in re-routing away from infected patients.
% In another study, Choi et al. \cite{choi2017large} use ML models for sentimental analysis to review public overreaction appearing in media articles and social media platforms. This type of in-depth analysis can rapidly monitor public reaction. It can also aid policy makers in taking the right actions in reducing fear and distress from the public regarding MERS.
% It is possible to predict the mortality rate patients that are infected with MERS. In study done \cite{turki2016greedy} a Greedy-Based Oversampling Approach (GBOA) integrated with ML classification models such as Random Forest (RF) and Support Vector Machine (SVM).
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{The socioeconomic impact of COVID-19, what can we determine so far using ML?}
% The virus spread across cities, provinces and countries worldwide. Forcing policy makers and regulators to take measures that would mitigate the spread of the virus. In Wuhan the city forced its residents to stay indoors, to shut down businesses and stop travel between other cities enforcing a city-wide lock-down on January 23rd \cite{qiu2020impacts}. These measures were necessary to control the spread of the virus, however, the actions were taken too late and the virus has now become a global pandemic. Nations around the world have since also followed the same and applied lock-down measures limiting person-to-person interactions. In this section we provide a summary of the impact COVID-19 has had on all of us as a society, and how the presence of the virus has caused an economic tremor. We attempt to connect to the best of our ability the ML research that has been done in presenting the socioeconomic impact of COVID-19 and how cities and policies will change.

% The world works in sync, there is plethora of trading that exists between countries. The manufacturing of an European car could take place in North America but the parts, tools and machinery used in the assembly could be shipped from Europe and Asia. Due to COVID-19 this global supply chain took a big hit which caused an economic disruption world-wide; \textit{Ali, I., et al.} \cite{ali2020covid} use a metaphorical example to explain the global supply-chain relating it to an actual steel chain, wherein, if any single link of the chain is damaged it would cause a hindrance and the reliability of the steel chain. Hence, China the largest exporter in the world \cite{jiang2020research} was unfortunately the origin of the global epidemic i.e. COVID-19 which created a devastating impact towards the world supply-chain. This has been an additional ripple effect towards other industries that were also effected by COVID-19. The production in the pharmaceutical industry in the US has slowed down as ingredients and equipment are imported from India and China. The revenues of the hospitality, aviation and travel industries have plummeted over the course of this pandemic which puts millions of jobs world-wide at risk \cite{nicola2020socio} \cite{evans2020socio}.
% The healthcare industry and the healthcare workers are at the front-lines in this battle against COVID-19 putting themselves in the most vulnerable position. In the aforementioned sections we have reviewed how ML related research may aid the healthcare workers but there is a change that is overdue in data-sharing practices. Data is very valuable especially medical data and maintaining the confidentiality and integrity is essential. \textit{Allam, Z., et al.} \cite{allam2020artificial} address how the cities are now transforming to smart cities that even more data is being collected and policy makers should alter some data-sharing policies. Having more access to location and communication data and integrating with ML and epidemiology models could aid in predicting future pandemics and making more rapid decisions that could mitigate and control the spread of an epidemic at the earliest. It is worth noting the fact that COVID-19 was evaluated as a potential pandemic in a mere days compared to SARS-CoV that took almost as long as a month.
% As policy makers have enforced lock-downs and societies have all been quarantining and maintaining social distance as an effort to mitigate the spread of COVID-19. 

% \textit{Dandekar, R., et al.} \cite{dandekar2020quantifying} use epidemiological equations with ML data-driven neural networks to assess how well these acts are controlling the spread of the virus.  
%%%%%%%%%%%%%%%%%%%%%%

% The term "Machine Learning" was first coined in 1959 by Arthur Samuel\cite{samuel1959some} in IBM with the concept of play checkers. As a subset of Artificial Intelligence(AI), Machine Learning(ML)\cite{el2015machine} is the technology that can imitate the human intelligence regarding its techniques without any programming necessity in various fields including finance\cite{laszlo2012machine}, industrial\cite{kashyap2017industrial}, eCommerce\cite{piramuthu2005machine}, medical\cite{magoulas1999machine}, and so on. Additionally, it is described as a performance optimizer by implementing example data or past mistakes\cite{alpaydin2020introduction}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%4

% In the \textit{First} phase, we review the role of ML in healthcare prior to the COVID-19 outbreak. We review the use of supervised learning and neural networks that can assist healthcare workers in diagnosing a patient for particular illnesses \cite{davenport2019potential} such as cancer.
% \textit{Second,} historic epidemics like Severe Acute Respiratory Syndrome (SARS-CoV) and Middle-East Respiratory Syndrome (MERS) are predecessors to COVID-19 \cite{andersen2020proximal}. We review the ML research that is done over those epidemics seeking whether those findings could be transferable to overcome the present day challenge of COVID-19.
% \textit{Three,} ML models models and algorithms trained on flight data, social media data, population density and epidemiological data can help in predicting outbreaks or provide signs of early warning. We review whether ML may have been able to predict the outbreak and forecast the spread of COVID-19.
% \textit{Fourth,} ML has the capability in assisting healthcare workers by aiding in speed testing and diagnosing compared to the traditional Reverse Transcription Polymerase Chain Reaction (RT-PCR) which can take up to 2 days in diagnosing \cite{mei2020artificial}; ML models have been used for image analysis in X-Rays and CT Scans in determining lung nodules, cancer and brain diagnosis \cite{suk2017deep} \cite{huang2017lung}. We review how ML algorithms can aid healthcare workers in detecting COVID-19 using such image classification models.
% \textit{Five,} there is still a shortage of any potential drug or vaccine that can fight the virus \cite{boldog2020risk} \cite{shereen2020covid}; we review the research of ML algorithms and models that is done over vaccine development. There are no present drugs that are available to fight the virus either \cite{zhou2020network} so it is essential to see whether current drugs could be re-purposed and whether ML can speed-up that process.
% \textit{Six,} we review the research that has been done over seeing how the coronavirus has impacted society and the social and economic impact it has made \cite{torales2020outbreak} \cite{fernandes2020economic}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Conclusion and Future Expectations}
% COVID-19 continues to spread at an alarming rate in some countries. The overall number of infected cases and the death toll both continue to rise with no signs of slowing down for countries. However, there are constant efforts being made by communities and domains to control the virus; the scientific and research community has surged towards finding a way to mitigate the spread of the virus and aiding in finding a cure. In this paper we review the efforts that are taken by the Machine Learning community to combat the virus. We reviewed how some ML based companies were able to provide early-warning signs and the use of such algorithms later also allow to forecast the spread over the course of the pandemic. ML based algorithms analyzing text over twitter are able to evaluate public sentiment over the course of this pandemic. ML algorithms can really aid healthcare workers and assist with diagnosis of the virus by using image classification techniques. ML based algorithms integrated with bioinformatics can also work towards evaluating how over-the-top counter drugs would react to the proteins of an infected COVID-19 patient. The review is inconclusive and as more research is being done on the topic it will be reviewed and added. For the future, we hope to see ML based programs that are modelled based from the findings of COVID-19. Models that can predict any future epidemics with much higher accuracy and for ML to be a tool that can act rapid enough to control the epidemic and stop it from turning into a global pandemic like COVID-19. 

%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Table-Code.tex <==
\begin{table*}[h!]
\begin{tabular}
{|l|c|c|c|c|}
\hline
  \multicolumn{1}{|c|}{Reference}&
  \multicolumn{1}{|c}{Sections}&
  \multicolumn{1}{|c}{Model and Technology}&
    \multicolumn{1}{|c|}{Description and Limitation}
  \\\hline
a &
  \multirow{4}{*}
  {Early Tracking, Prevention}
 & potato & fried \\\cline{3-4}
b & &  potato & fried jacket\\\cline{3-4}
c & & \\\cline{3-4}
d & & \\\cline{3-4} \hline
k &
  \multirow{4}{*}
  {Forecasting}
 & potato & fried \\\cline{3-4}
b & & jacket\\\cline{1-1}
c & & \\\cline{1-1}
d & & \\\cline{1-1}\hline
z &
  \multirow{4}{*}
  {Tracking}
 & potato & fried \\\cline{3-4}
b & & jacket\\\cline{1-1}
c & & \\\cline{1-1}
d & & \\\cline{1-1}
\hline
\end{tabular}
\end{table*}

==> Table_2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}
% \centering
%   \caption{\label{tab:table-name} ML Research done towards Diagnosing COVID-19.}
%   \begin{tabular}{|m{3cm} | m{1.5cm} | m{3cm}| m{4cm} | m{5cm}|}  
%  \hline
%  \textbf{Ref} & \textbf{Image Type} & \textbf{Dataset} & \textbf{Methods} & \textbf{Remarks} \\ [0.5ex] 
%  \hline

% \cite{apostolopoulos2020covid} & \multirow{11}{*}{X-Ray} &  Multiple curated Datasets \textit{source: Github} & DL - CNN, Feature Extraction (various models) & Various model performance comparison  \\ \cline{1-1}\cline{3-5}
% \cite{ghoshal2020estimating} &                   & Publicly available Chest X-Ray Images & Bayesian Deep Learning Classifiers & Using Transfer learning approach with the classifier to estimate uncertainty. \\  \cline{1-1}\cline{3-5}
%  \cite{farooq2020covid}, \cite{wang2020covid}, \cite{ucar2020covidiagnosis}, \cite{afshar2020covid}, \cite{luz2020towards}, \cite{khobahi2020coronet}, \cite{sarker2020covid}, \cite{hirano2020vulnerability}, \cite{hemdan2020covidx} &                   & COVIDx & Multiple prepossessing techniques like normalization integrated with various deep neural works and classifiers  & \begin{itemize} 
%  \item\cite{khobahi2020coronet} \cite{sarker2020covid} \cite{luz2020towards} \cite{wang2020covid} multiple approaches like semi-supervised approach, feature extraction and transfer learning methodology implemented.
%  \item\cite{ucar2020covidiagnosis} present an AI system that  classifies input of X-Ray images of Normal, COVID-19, Pneumonia using DL.
%  \item\cite{farooq2020covid} Use a ResNet classifier to achieve excellent classification accuracy.
%  \item\cite{hemdan2020covidx} Test and train multiple image classifiers to obtain the highest accuracy identifying the virus. VGG19 and DenseNet have a high accuracy score.
%  \item \cite{hirano2020vulnerability} Demonstrate how DNNs are vulnerable to a universal adversarial perturbation causing failure in classification tasks, fine-tuning may be able to improve this. 
%  \item \cite{afshar2020covid} An alternative modeling framework based on Capsule Networks.
% %  \item \cite{sarker2020covid} Clear explanation of how model works using a novel transfer learning approach 
%  \end{itemize} \\ \cline{1-1}\cline{3-5}
% \cite{narin2020automatic} &                   & Small Dataset available on GitHub & Three different CNN models (InceptionV3, ResNet50, Inception-ResNetV2) & ResNet50 provides the highest classification. \\ \cline{1-1}\cline{3-5}
% \cite{maghdid2020diagnosing} &                   & Multiple Sources & Modified Pre-trained AlexNet and a simple CNN & Pre-Trained network achieves a higher accuracy  \\ \cline{1-1}\cline{3-5}
% \cite{tougaccar2020covid} &                   & Multiple Sources and Datasets & MobileNetV2/SqueezeNet & They use DL models achieve high classification rate\\ \cline{1-1}\cline{3-5}
% \cite{ozturk2020automated} &                   & Multiple Sources  & DarkCovidNet (CNN) & Provides two approaches, a binary classification and multi-class classification. Binary model performs better and higher\\ \cline{1-1}\cline{3-5}
% \cite{rajaraman2020training} &                   & Multiple sources, datasets & VGG16, InceptionV3, Xception, DenseNet-121, NasNet-Mobile, etc models compared & VGG16 achieved the highest rate\\ \cline{1-1}\cline{3-5}
% \cite{jamil2020automatic} &                   & Kaggle Repository & Convolutional Neural Network & The authors are able to get 93\% accuracy \\ \cline{1-1}\cline{3-5}
% \cite{sethy2020detection} &                   & Multiple Datasets & Trained 9 different models for COVID-19 & ResNet50 + SVM achieved the highest accuracy\\ \cline{1-1}\cline{3-5}
%     \cite{panwar2020application}  &                   & COVID-19 + Normal XRay images & nCOVnet(VGG-16) & The proposed model is able to achieve high accruacy in predicting COVID-19 infected patients from CXR Images \\ \cline{1-1} \cline{3-5}
% \cite{apostolopoulos2020extracting} &                   & Multiple Datasets & MobileNetV2 & Training the CNN MobileNetV2 model from scratch proves to get higher accuracy compared to transfer learning techniques  \\ \cline{1-6}
% \hline
%  \cite{zhao2020covid}  & \multirow{15}{*}{CT-Scan} & Open-sourced COVID-CT \textit{source: Github} & multi-task and self-supervised learning & Clinically useful.   \\ \cline{1-1} \cline{3-5} 
%   \cite{tang2020severity} &                   & Clinical CT Images of 176 & Random Forest / three-fold cross-validation & The Random Forest model showing promising performance towards reflecting the severity of COVID-19 \\ \cline{1-1} \cline{3-5}
%  \cite{gozes2020rapid} &                   &   Multiple Datasets \textit{Multiple Source: Hospitals / Chainz} & ResNet50 & High accuracy in identifying whether COVID-19 cases \\ \cline{1-1} \cline{3-5}
%   \cite{li2020artificial} &                   & Independent Dataset CT Images & Present a Deep Learning model CovNET & The model has the ability to high accuracy in identify COVID-19 cases from other lung diseases  \\ \cline{1-1} \cline{3-5}
%     \cite{butt2020deep}  &                   &  Clinical CT Scan Images & Deep Learning - ResNet18 & Using a location attention mechanism on the model distinguishes COVID-19 cases from others with higher accuracy \\ \cline{1-1} \cline{3-5}
%     \cite{wang2020deep} &                   &   CT Scan Images Dataset, Clinical &  Modified Transfer Learning - Inception Model & Use a fine-tuning technique with pre-trained weights \\ \cline{1-1} \cline{3-5}
%         \cite{bai2020predicting} &                   &  China Health Commission Dataset, etc & Multi Stage - DL Models, LSTM & The model is capable of extracting spatial and temporal information efficiently thereby improving prediction performance \\ \cline{1-1} \cline{3-5}
%       \cite{pathak2020deep}  &                   & Multiple datasets  & ResNet50 & The model with transfer learning technique performs better than alternative supervised learning methods \\ \cline{1-1}        \cline{3-5}
%         \cite{jin2020ai}  &                   &  Multiple sources: Hospitals & Various DL learning models (Inception, ResNet50, 3D U-Net++) & Able to deploy the model in 4 weeks overcoming challenges and achieving a high accuracy rate\\    \cline{1-1} \cline{3-5}
%         \cite{shan2020lung}  &                   & Clinical Dataset & Deep Learning - VB-Net & Introducing a Human-in the loop section to refine automation of each case - the model can segment and quantify infected regions\\ \cline{1-1} \cline{3-5}
%     \cite{wang2020noise}  &                   & Clinical Dataset & COPLE-Net + Noise-Robust Dice Loss & The technique presented outperforms standard Noise-Robust loss functions, COPLE-Net and the framework both perform quite highly in segmenting labels for COVID-19 pneumonia lesion\\ \cline{1-1} \cline{3-5}
%         \cite{song2020end}  &                   & Clinical Dataset (China) & BigBiGAN (bi-directional generative adversarial network) & The model achieves high validation accuracy in identifying COVID-19 pneumonia from CT images\\ \cline{1-1} \cline{3-5}
%         \cite{yang2020end}  &                   & COVID-19, Normal pneumonia and regular CXR & Inception V1 & Validate the model in 3 ways including 10-fold cross-validation achieving high AUC for the validation dataset \\ \cline{1-1} \cline{3-5}
%         \cite{zheng2020deep} &                   &  Clinical & UNet, Weakly Supervised DL Network (DeCovNet)  & Accurately predict COVID-19 infectious probability without annotating lesions for training  \\  \cline{1-6}
%   \hline
%  \end{tabular}
% \end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\centering
  \caption{\label{tab:table-name} ML Research done towards Diagnosing COVID-19.}
%   \begin{tabular}{|m{3cm} | m{1.5cm} | m{3cm}| m{4cm} | m{5cm}|}  
 \begin{adjustbox}{width=\textwidth}
 \begin{tabular}{m{3cm}  m{1.5cm}  m{3cm} m{4cm} m{5cm}} 
 \hline
 \textbf{Ref} & \textbf{Image Type} & \textbf{Dataset} & \textbf{Methods} & \textbf{Remarks} \\ [0.5ex] 
 \hline

\cite{apostolopoulos2020covid} & \multirow{11}{*}{X-Ray} &  Multiple curated Datasets \textit{source: Github} & DL - CNN, Feature Extraction (various models) & Various model performance comparison  \\ \cline{1-1}\cline{3-5}
\cite{ghoshal2020estimating} &                   & Publicly available Chest X-Ray Images & Bayesian Deep Learning Classifiers & Using Transfer learning approach with the classifier to estimate uncertainty \\  \cline{1-1}\cline{3-5}
 \cite{farooq2020covid}, \cite{wang2020covid}, \cite{ucar2020covidiagnosis}, \cite{afshar2020covid}, \cite{luz2020towards}, \cite{khobahi2020coronet}, \cite{sarker2020covid}, \cite{hirano2020vulnerability}, \cite{hemdan2020covidx} &                   & COVIDx & Multiple prepossessing techniques like normalization integrated with various deep neural works and classifiers  & \begin{itemize} 
 \item\cite{khobahi2020coronet} \cite{sarker2020covid} \cite{luz2020towards} \cite{wang2020covid} multiple approaches like semi-supervised approach, feature extraction and transfer learning methodology implemented.
 \item\cite{ucar2020covidiagnosis} present an AI system that  classifies input of X-Ray images of Normal, COVID-19, Pneumonia using DL.
 \item\cite{farooq2020covid} Use a ResNet classifier to achieve excellent classification accuracy.
 \item\cite{hemdan2020covidx} Test and train multiple image classifiers to obtain the highest accuracy identifying the virus. VGG19 and DenseNet have a high accuracy score.
 \item \cite{hirano2020vulnerability} Demonstrate how DNNs are vulnerable to a universal adversarial perturbation causing failure in classification tasks, fine-tuning may be able to improve this. 
 \item \cite{afshar2020covid} An alternative modeling framework based on Capsule Networks.
%  \item \cite{sarker2020covid} Clear explanation of how model works using a novel transfer learning approach 
 \end{itemize} \\ \cline{1-1}\cline{3-5}
\cite{narin2020automatic} &                   & Small Dataset available on GitHub & Three different CNN models (InceptionV3, ResNet50, Inception-ResNetV2) & ResNet50 provides the highest classification. \\ \cline{1-1}\cline{3-5}
\cite{maghdid2020diagnosing} &                   & Multiple Sources & Modified Pre-trained AlexNet and a simple CNN & Pre-Trained network achieves a higher accuracy  \\ \cline{1-1}\cline{3-5}
\cite{tougaccar2020covid} &                   & Multiple Sources and Datasets & MobileNetV2/SqueezeNet & They use DL models achieve high classification rate\\ \cline{1-1}\cline{3-5}
\cite{ozturk2020automated} &                   & Multiple Sources  & DarkCovidNet (CNN) & Provides two approaches, a binary classification and multi-class classification. Binary model performs better and higher\\ \cline{1-1}\cline{3-5}
\cite{rajaraman2020training} &                   & Multiple sources, datasets & VGG16, InceptionV3, Xception, DenseNet-121, NasNet-Mobile, etc models compared & VGG16 achieved the highest rate\\ \cline{1-1}\cline{3-5}
\cite{jamil2020automatic} &                   & Kaggle Repository & Convolutional Neural Network & The authors are able to get 93\% accuracy \\ \cline{1-1}\cline{3-5}
\cite{sethy2020detection} &                   & Multiple Datasets & Trained 9 different models for COVID-19 & ResNet50 + SVM achieved the highest accuracy\\ \cline{1-1}\cline{3-5}
    \cite{panwar2020application}  &                   & COVID-19 + Normal XRay images & nCOVnet(VGG-16) & The proposed model is able to achieve high accruacy in predicting COVID-19 infected patients from CXR Images \\ \cline{1-1} \cline{3-5}
\cite{apostolopoulos2020extracting} &                   & Multiple Datasets & MobileNetV2 & Training the CNN MobileNetV2 model from scratch proves to get higher accuracy compared to transfer learning techniques  \\ \cline{1-6}
\hline
 \cite{zhao2020covid}  & \multirow{15}{*}{CT-Scan} & Open-sourced COVID-CT \textit{source: Github} & multi-task and self-supervised learning & Clinically useful.   \\ \cline{1-1} \cline{3-5} 
  \cite{tang2020severity} &                   & Clinical CT Images of 176 & Random Forest / three-fold cross-validation & The Random Forest model showing promising performance towards reflecting the severity of COVID-19 \\ \cline{1-1} \cline{3-5}
 \cite{gozes2020rapid} &                   &   Multiple Datasets \textit{Multiple Source: Hospitals / Chainz} & ResNet50 & High accuracy in identifying whether COVID-19 cases \\ \cline{1-1} \cline{3-5}
  \cite{li2020artificial} &                   & Independent Dataset CT Images & Present a Deep Learning model CovNET & The model has the ability to high accuracy in identify COVID-19 cases from other lung diseases  \\ \cline{1-1} \cline{3-5}
    \cite{butt2020deep}  &                   &  Clinical CT Scan Images & Deep Learning - ResNet18 & Using a location attention mechanism on the model distinguishes COVID-19 cases from others with higher accuracy \\ \cline{1-1} \cline{3-5}
    \cite{wang2020deep} &                   &   CT Scan Images Dataset, Clinical &  Modified Transfer Learning - Inception Model & Use a fine-tuning technique with pre-trained weights \\ \cline{1-1} \cline{3-5}
        \cite{bai2020predicting} &                   &  China Health Commission Dataset, etc & Multi Stage - DL Models, LSTM & The model is capable of extracting spatial and temporal information efficiently thereby improving prediction performance \\ \cline{1-1} \cline{3-5}
      \cite{pathak2020deep}  &                   & Multiple datasets  & ResNet50 & The model with transfer learning technique performs better than alternative supervised learning methods \\ \cline{1-1}        \cline{3-5}
        \cite{jin2020ai}  &                   &  Multiple sources: Hospitals & Various DL learning models (Inception, ResNet50, 3D U-Net++) & Able to deploy the model in 4 weeks overcoming challenges and achieving a high accuracy rate\\    \cline{1-1} \cline{3-5}
        \cite{shan2020lung}  &                   & Clinical Dataset & Deep Learning - VB-Net & Introducing a Human-in the loop section to refine automation of each case - the model can segment and quantify infected regions\\ \cline{1-1} \cline{3-5}
    \cite{wang2020noise}  &                   & Clinical Dataset & COPLE-Net + Noise-Robust Dice Loss & The technique presented outperforms standard Noise-Robust loss functions, COPLE-Net and the framework both perform quite highly in segmenting labels for COVID-19 pneumonia lesion\\ \cline{1-1} \cline{3-5}
        \cite{song2020end}  &                   & Clinical Dataset (China) & BigBiGAN (bi-directional generative adversarial network) & The model achieves high validation accuracy in identifying COVID-19 pneumonia from CT images\\ \cline{1-1} \cline{3-5}
        \cite{yang2020end}  &                   & COVID-19, Normal pneumonia and regular CXR & Inception V1 & Validate the model in 3 ways including 10-fold cross-validation achieving high AUC for the validation dataset \\ \cline{1-1} \cline{3-5}
        \cite{zheng2020deep} &                   &  Clinical & UNet, Weakly Supervised DL Network (DeCovNet)  & Accurately predict COVID-19 infectious probability without annotating lesions for training  \\  \cline{1-6}
  \hline
 \end{tabular}
\end{adjustbox}
\end{table*}
